Answering Questions by Meta-Reasoning over Multiple Chains of Thought

Modern systems for multi-hop question answering (QA) typically break questions into a sequence of reasoning steps, termed chain-of-thought (CoT), before arriving at a final answer. Often, multiple chains are sampled and aggregated through a voting mechanism over the final answers, but the intermediate steps themselves are discarded. While such approaches improve performance, they do not consider the relations between intermediate steps across chains and do not provide a unified explanation for the predicted answer. We introduce Multi-Chain Reasoning (MCR), an approach which prompts large language models to meta-reason over multiple chains of thought, rather than aggregating their answers. MCR examines different reasoning chains, mixes information between them and selects the most relevant facts in generating an explanation and predicting the answer. MCR outperforms strong baselines on 7 multi-hop QA datasets. Moreover, our analysis reveals that MCR explanations exhibit high quality, enabling humans to verify its answers.

==> old_01_intro.tex <==
\section{Introduction}
\label{sec:introduction}

% Today there is a standard way for handling reasoning in LLMs: chain of thought to elicit reasoning often combined with retrieval for less hallucination 


% Moreover, it has been shown that one can use multiple chains of thought and aggregate over them through simple majority voting and that is the best there is right now more or less.

Large language models (LLMs) such as GPT-3 \cite{NEURIPS2020_1457c0d6} \jb{in this day and age citing only OpenAI seems problematic need more diversity. No need to mention GPT-3 in my opinion but cite also palm, anthropic, LLama, Eleuther?} have demonstrated remarkable performance on a wide range of natural language tasks. In order \jb{9 out of 10 times you can omit the `in order'} to elicit multi-step reasoning in LLMs, \citet{Wei2022ChainOT} proposed \emph{chain-of-thought} (CoT) prompting, which demonstrates to the model how to solve problems step-by-step. This method is often extended to open-domain tasks by incorporating a \emph{retrieval} component \cite{press2023measuring, trivedi2022interleaving, Khattab2022DemonstrateSearchPredictCR}.
Incorporating retrieval assists LLMs which may be prone to hallucination or struggle to represent the full long tail of knowledge from their training corpus.
% \oy{maybe we can add that retrieval also assists in places where info is not encoded in the model's params?}
\jb{this can still be compressed / be made more targeted. I don't think there is a need for one sentence on LLMs in general and one sentence on CoT. I think the first sentence can talk about reasoning with LLMs immediately and cite mention LLMs in general in passing. This immediately points that this paper is about reasoning with LLMs, current first sentence is too generic}
\jb{now the second sentence is about retrieval -- but maybe it's not needed at all at this point? it's in the way between introdcuing cot and talking about multiple chains. So So potentially you can have one paragraph about cot and sc and then immediately have a paragraph talking about their problems - one problem not mentioned is that if the output space is large majority will just be uniform across many answers? Then perhaps the whole thing about retrieval can be in a background section and not in the intro following the intro? right now the retrieval is not necessaritly helpful for understanding things. If it's needed then where? maybe for the figure? maybe it can be introduced more succinctly?}


% say what is the problem with this - why is SC problematic. 

\citet{wang2023selfconsistency} further expanded the CoT framework, introducing the \emph{self-consistency} (SC) method. They have shown that CoT accuracy can be improved by sampling multiple chains of thought and aggregating over their answers using simple majority voting \jb{writing can be compressed, see comment above about being more targeted}. 
While self-consistency has lead to significant gains, the approach has several shortcomings.\uk{Isn't it too early to start saying "ours is better"?} As \selfconsistency{} relies on sampling multiple reasoning chains, some of these may potentially end in incorrect answers \jb{this seems trivial so the point is in the next sentence maybe there's a better way to write this}. By focusing entirely on the final answers, \selfconsistency{} ignores all the information that is present in the intermediate reasoning steps of the chain. These steps may contain relevant information, even though their final answer may be wrong. For example, in Fig.~\ref{fig:multi_chain_example}, reasoning chain \#2 has a wrong answer however, its steps provide highly relevant information (\textit{``What is a Yeti?''}, \textit{``What are prehensile limbs?''}).
Another shortcoming of \selfconsistency{} concerns its relative opaqueness compared to the original CoT method. By returning the majority vote on multiple answers, it lacks any readable explanation of its final result, and in contrast to CoT. \oy{maybe we can add here that: (1) all chains that lead to the same label have the same weight, although some of them may be incorrect (2) that it can't account to synonyms and is unclear how to use for open-ended answers and (3) that it incurs high cost } \bb{yes, add more disadvantages} \jb{isn't one that if the output is very open-domain you easily get ties?}

\begin{figure}[t]\setlength{\belowcaptionskip}{-8pt}
  \centering
  \includegraphics[trim={0cm 19cm 4.1cm 0cm}, clip, width=0.49\textwidth]{figures/fig_1.pdf}
  \vspace*{-0.7cm}
  \caption{Answering a question with multiple chains of thought serving as the QA model`s context. \oy{I think we can make this a bit nicer visually (crossing arrows), more important if people think this is a good example that tells the story well.}\uk{really like the design, colors etc, but the amount of text is overwhelming and it wont be readable for a printed version of the paper, you need to zoom-in a-lot to read it..}}
  \label{fig:multi_chain_example}
\end{figure}


% then say that in this work we present an approach that falls under the general paradigm of cot+retrieval+aggregate but uses a different approach for aggregation specifically uses entailment or reading comprehension we need to decide what makes more sense. Basically we add another model that is an LLM with prompt for doing this aggregation. This should be accompanied by referencing figure 1 where you really nail the point why entailment is better than SC.

In this work we present a new method for reasoning over multiple chains of thought \bb{say the gist of the diff already in the first sentence} \jb{+1} \jb{A sentence that might be nice to have somewhere maybe here is `We use cot not to generate \emph{answers} but instead to \emph{collect pieces of evidence} or sth like that. I think we should frame contribution in a way that is interesting and insightful and this might be one.}. Our approach follows the same \jb{delete `same'} paradigm of chain-of-thought reasoning combined with retrieval \jb{does retrieval matter here?}, in order to answer multi-hop open-domain questions. 
Given multiple reasoning chains, we differ from \selfconsistency{}, and instead use a prompted LLM to jointly reason over all chains and generate the final answer.
Fig.~\ref{fig:multi_chain_example} directly compares our Multi-Chain-Entailment (\mte{}) approach with that of \selfconsistency{}. First, both methods rely on multiple reasoning chains that are sampled from a \decomposition{} model (e.g., a CoT-prompted LLM) \bb{probably better to avoid referring to the models before defining them better - if unavoidable maybe add "decomposition model" to figure 1} \jb{yes don't refer to something unnamed, you can say it's an LLM-based thing, somewhere this needs mentioning that this is not a trained module}. \selfconsistency{} will then return the majority answer, based on the answers of all sampled chains (grey box to the right). By contrast, \mte{} concatenates the intermediate facts from each chain into a unified context (pink box to the left). This context, along with the original question, are then fed to a separate \entailment{} model. The \entailment{} model is an LLM which is prompted, CoT-style, to answer the original question based on its input context. It generates a detailed CoT explanation, followed by the final result (pink box to the right).
By substituting \selfconsistency{} with a prompted LLM we enable \mte{} to be more expressive \jb{increase expressivity}, both in terms of its multi-chain aggregation \jb{opaque term}, as well as its output CoT explanation. \bb{somewhere in this paragraph emphasize why this is desired - e.g. we may want the component to override majority, combine facts, etc.}  \jb{why is entailment ok then? didn't we say rc is more appropriate? need to discuss...}



%%%%%%%%%%%%%%%%%%%%

\mte{} is comprised of three main components \S\ref{sec:method}. The first two components are a \decomposition{} and \retriever{} which jointly generate the reasoning chain (Fig~\ref{fig:architecture}) \jb{this is perhaps the only place you need retrieval in intro?}. The chain is comprised of intermediate questions and answers, generated by the \decomposition{} model along with intermediate contexts provided by the \retriever{} \cite{trivedi2022interleaving}. The third component is aforementioned \entailment{} model for multi-chain aggregation. 
In Fig.~\ref{fig:multi_chain_example} we describe how \mte{} utilizes multiple reasoning chains.
Given the question \textit{``Would a Yeti be likely to have prehensile limbs?''} we initially sample 3 reasoning chains using the \decomposition{} model and our \retriever{}. We then concatenate the intermediate questions and answers from each chain, formatting them as a list of statements. This context is then fed to our \entailment{} LLM, prompted for reading comprehension in CoT format. The output is then a short explanation followed by the final answer to the question. 
Specifically, the \entailment{} is prompted to read the context and extract evidence facts to serve as its CoT explanation.
Note that in its answer explanation \mte{} combines facts from two different reasoning chains: (1) \textit{``Yeti is a mythical ape like creature...''}; (2) \textit{``Large apes ... have prehensile limbs''}. 
Compared to self-consistency, \mte{} reasons over full chains and is therefore able to combine facts from different ones. Additionally, as it is exposed to facts from multiple chains, \mte{} has the potential to select the facts which are best supported by all reasoning chains. \uk{does your experiment support this claim? (the second claim, after additionally)}
% We consider these as clear advantages in open-domain tasks such as information-seeking QA or fact verification. Furthermore, \mte{} provides a human-readable explanation that can traced back to its reasoning chains and potentially to the retrieved contexts \cite{Bohnet2022AttributedQA}. 
%This contrasts the relative opaqueness of SC that outputs the final answer based on majority voting.

We evaluate \mte{} on \numdatasets{} multi-hop datasets in an open-domain setting. We distinguish between tasks based on their reasoning type. \bb{Why is it important to distinguish the two types? Maybe emphasize that we want a system that would work well on both, but that this is not trivial?}\uk{imo its good to emphasize the diversity of datasets and task to show MTE handle different QA reasoning types } Implicit reasoning tasks entail implicit reasoning steps, which cannot be explicitly derived from the original question \cite{tafjord-etal-2019-quartz, geva-etal-2021-aristotle,kalyan-etal-2021-much}. Explicit reasoning tasks have a single reasoning strategy, clearly expressed in the question \cite{yang2018hotpotqa, welbl2018constructing, press2023measuring, Aly2021FEVEROUSFE}. As our baselines we compare \mte{} to SC, as well as implemented variants of the Self-Ask \cite{press2023measuring} as well as CoT augmented with context-based retrieval, similar to \cite{trivedi2022interleaving}. Overall, we observe that \mte{} outperforms all other baselines (\S\ref{sec:experiments}). In particular beating SC where both make use of the same reasoning chains. In \S\ref{sec:analysis} we provide a quantitative analysis of the benefits of reasoning over multiple CoTs. In addition we qualitatively score the explanations generated by \mte{} and estimate their accuracy. 
Following an extensive error analysis, we find that our system generates high quality explanations \bb{add number}. Last, we analyze the performance of each individual component in our modular approach and provide insights into potential improvements.

Our main contributions are as follows:

\begin{itemize}
  \item Introducing the \mte{} method for open-domain QA, by reasoning over multiple chains of thought. Replacing, the majority vote of self-consistency with a prompted \entailment{} model.
  \item Evaluating our method on \numdatasets{} benchmarks for multi-hop open-domain question answering, showing it outperforms self-consistency. \oy{I think it might be nicer to say in point one that we suggest this to ODQA, and then in point 2 highlight the empirical results and analysis?}\bb{I agree}
\end{itemize}
Our codebase and prompts are publicly available.\footnote{\url{https://github.com/XXX}}
\oy{In terms of previous work: do we think that verifiers/diverse paper are relevant? I guess not for intro...}\bb{I agree} \jb{Since the space is so dense I do wonder if a short background section will help layout terminology and mention very related work upfront}


%%% TW - old version

% Large language models (LLMs) such as GPT-3 \cite{NEURIPS2020_1457c0d6} have demonstrated remarkable performance on a wide range of natural language tasks. However, recent works have highlighted the shortcoming of LLMs on tasks that require multiple steps of reasoning \cite{Zhou2022LeasttoMostPE, press2023measuring}. In order to unlock multi-step reasoning in LLMs \citet{Wei2022ChainOT} proposed \emph{chain-of-thought} (CoT) prompting, by demonstrating to the model how to solve problems step-by-step. \citet{wang2023selfconsistency} further expanded the CoT framework by introducing the \emph{self-consistency} (SC) method. SC proposes a ``sample-and-marginalize'' approach, sampling multiple reasoning chains from the LLM, then marginalizing over them and returning the majority answer. SC has been shown to outperform CoT on arithmetic and commonsense tasks, beating other approaches such as verifying or re-ranking sampled reasoning chains \cite{cobbe2021training, Thoppilan2022LaMDALM}. \oy{I think they also have HotpotQA in the SC paper. Maybe we can just say that SC has been proposed to aggregate info from multiple chains for QA, outperforming previous approaches?}.
% Originally, these approaches have been applied to questions whose relevant information was either provided in context (arithmetic problems) or was present in the model parameters (commonsense questions). However, when tackling open-domain questions LLMs may be prone to hallucination and cannot represent the full long tail of
% knowledge from the training corpus. Therefore, recent works proposed integrating a \emph{retrieval} component into CoT prompting \cite{press2023measuring, trivedi2022interleaving, Khattab2022DemonstrateSearchPredictCR}, interleaving the reasoning and retrieval steps. 

% In this work we present an approach that reasons on multiple reasoning chains to answer multi-hop open-domain questions. Rather than taking the majority answer of multiple chains, as in SC, we prompt an LLM to reason on these chains and generate the answer. The approach is somewhat akin to performing CoT reasoning where the context is itself comprised of multiple chains of thought. Our Multi-Chain-Entailment (\mte{}) is comprised of three main components \S\ref{sec:method}. The first two components are a \decomposition{} and \retriever{} which jointly generate the reasoning chain. The reasoning chain is comprised of intermediate questions and answers, generated by the \decomposition{} model along with intermediate contexts provided by the \retriever{} \cite{trivedi2022interleaving}. The third component is our \entailment{} model which receives as input multiple reasoning, sampled from the \decomposition{} model, and deduces the final answer to the question. 
% In Fig. \ref{fig:multi_chain_example} we describe how \mte{} utilizes multiple reasoning chains.
% Given the question \textit{``Would a Yeti be likely to have prehensile limbs?''} we initially sample 5 reasoning chains using the \decomposition{} model and our \retriever{}. We then concatenate the intermediate questions and answers from each chain, formatting them as a list of statements. This context is then fed to our \entailment{} LLM, prompted for reading comprehension in CoT format. The output is then a short explanation followed by the final answer to the question. Note that in its answer explanation \mte{} combines facts from two different reasoning chains: (1) \textit{``Yeti is a mythical ape like creature...''}; (2) \textit{``Large apes ... have prehensile limbs''}. 
% Compared to self-consistency, \mte{} performs inter-CoT reasoning and is therefore able to combine facts from different chains. Additionally, as it is exposed to facts from multiple chains, \mte{} has the potential to select the facts which are best supported by all reasoning chains. 
% We consider these as clear advantages in open-domain tasks such as information-seeking QA or fact verification. Furthermore, \mte{} provides a human-readable explanation that can traced back to its reasoning chains and potentially to the retrieved contexts \cite{Bohnet2022AttributedQA}. This contrasts the relative opaqueness of SC that outputs the final answer based on majority voting.

% We evaluate \mte{} on \numdatasets{} multi-hop datasets in an open-domain setting. These tasks require commonsense reasoning \cite{tafjord-etal-2019-quartz, geva-etal-2021-aristotle,kalyan-etal-2021-much}, information seeking \cite{yang2018hotpotqa, welbl2018constructing, press2023measuring} and fact-verification \cite{Aly2021FEVEROUSFE}. As our baselines we compare \mte{} to SC, as well as implemented variants of the Self-Ask \cite{press2023measuring} as well as CoT augmented with context-based retrieval, similar to \cite{trivedi2022interleaving}. Overall, we observe that \mte{} outperforms all other baselines (\S\ref{sec:experiments}). In particular beating SC where both make use of the same reasoning chains. In \S\ref{sec:analysis} we provide a quantitative analysis of the benefits of reasoning over multiple CoTs. In addition we qualitatively score the explanations generated by \mte{} and estimate their accuracy. 
% Following an extensive error analysis, we find that our system generates high quality explanations. We further analyze the performance of each individual component in our modular approach.

% Our main contributions are as follows:

% \begin{itemize}
%   \item Introducing the \mte{} method for reasoning over multiple chains of thought, separating between the \decomposition{} and answer \entailment{} components.
%   \item Evaluating our method on \numdatasets{} benchmarks for multi-hop open-domain question answering, showing it outperforms self-consistency.
% \end{itemize}
% Our codebase and prompts are publicly available.\footnote{\url{https://github.com/XXX}}


==> old_03_method.tex <==
\section{Method}
\label{sec:method}

We present a method for answering questions by reasoning over multiple chains of thought. Our focus is on  open-domain question answering, where the input is a question $q$, such that the evidence to answer it exists in one or more facts in a corpus $C$ \jb{is this notation used anywhere later?}.
As answering $q$ may entail \jb{require} multiple \jb{reasoning?} steps, it \jb{what is `it'?} can be expressed by a \emph{question decomposition} denoted by $d$. The decomposition is a list of one or more intermediate question-context-answer tuples $(q_i, c_i, a_i)$ \jb{what is `a context'? how does one get it?}.
Thus, $d$ constitutes a reasoning chain of steps for solving $q$.
Fig.~\ref{fig:architecture} describes our approach. Given the question \textit{``How many ants would fit in The Shard?''}. In steps 1-2, we generate multiple reasoning chains \jb{there is use of both `question decomposition` and `reasoning chain'. are they different? if so how? if yes, do we need both? and if we need we should say they are the same}, $d^{(1)},...,d^{(k)}$. Each $d^{(j)}$ is iteratively generated by interleaving generated intermediate questions with retrieved contexts (\S\ref{sec:method_decomp_retrieve}). Our main contribution is in step 3, which introduces an \entailment{} step over multiple sampled decompositions (\S\ref{sec:method_entail}). 

\jb{where do we say that all these models are not trained and are prompted language models? we need to do this somewhere. Moreover since they are defined by the prompt - we should say what is the prompt right? or describe it and say something about it and where we have it exactly? basically a model is a combination of parameters+prompt.}

\begin{figure*}[t]\setlength{\belowcaptionskip}{-8pt}
  \centering
  \includegraphics[trim={0cm 0cm 0.5cm 0cm}, clip, width=\textwidth]{figures/fig_system_overview.pdf}
  \vspace*{-0.7cm}
  \caption{An overview of \mte{}. Given a multi-hop question steps 1-2 generate multiple reasoning chains by conditioning the generation of intermediate questions and answers on retrieved evidence sentences. In step 3 the \entailment{} model generates the final answer, conditioned on multiple reasoning chains from the previous steps. \oy{Maybe it's best to have an example without contradicting facts?}}
  \label{fig:architecture}
\end{figure*}

\subsection{Decomposition and Retrieval}
\label{sec:method_decomp_retrieve}
Given an open-domain question $q$, we generate its reasoning chain \jb{so not question decomposition?} with two models: (1) the \decomposition{} model, and (2) the \retriever{}. 

\paragraph{Decomposition.} The \decomposition{} model receives $q$ and generates a list of intermediate question-answer pairs $(q_i, a_i)$ ending in the final answer to $q$. Our decomposition format is \emph{Self-Ask} \cite{press2023measuring}, which generates explicit intermediate questions, unlike  chain-of-thought  \cite{Wei2022ChainOT} \jb{which is what? also why?}. Fig.~\ref{fig:architecture} presents example reasoning chains, preceded by retrieved contexts (see below) and ending with the final answer to $q$. \jb{I don't understand it seems this is something that we never do but here it seems we do do this so confusing.}

\paragraph{Retrieval.} The \retriever{} receives an intermediate question $q_i$ and returns sentences $c_i \in C$ used as relevant contexts to answer $q_i$. We incorporate the retrieved contexts in our \decomposition{} model, following the method of \citet{trivedi2022interleaving}. Fig.~\ref{fig:decompose_retrieve} describes our interleaving of decomposition and retrieval steps. First, the \decomposition{} model generates the entire reasoning chain, sans retrieval. However, only the first intermediate question, $Q_1$ is kept and is used as input to the first retrieval step (in yellow). We then prepend the retrieved context $C_1$ and use the \decomposition{} to generate intermediate answer $A_1$. This is followed by generating the next intermediate question $Q_2$, and so forth. Note that we prepend intermediate contexts to the beginning of the chain instead of interleaving them as in \cite{press2023measuring}. We observe this significantly boosts the decomposition accuracy in returning the final answer $a$. 
\jb{IIUC, you use the decomposition model to generate the question and answers and apply it again and again but with contexts - right no it's confusing because it seems we do full decomposition but then we change the description. I think some thought is required here how to describe this more cleanly maybe no need to separate to two paragraph of retrieval and decomposition, just expalin their roles, say that decomposition generates questions, retrieval retrieves context and decomposition also generates answers based on context or sth.}


\subsection{Entailment on Multiple Reasoning Chains}
\label{sec:method_entail}

\jb{add starting sentence that re-groups the reader, this starts very abruptly for the main point of the paper. again here you can repeat use of cot for context generation and not answering.}

The \entailment{} model is tasked with reasoning on multiple chains of thought in order to answer $q$ \bb{perhaps say again that this is the focus, and give again a short motivation for the component} \jb{+1}. First, we sample a diverse set of reasoning chains $d^{(1)}...d^{(k)}$ from the \decomposition{} model \jb{not the retriever? maybe there should be name for first part that combines decomposition and retrieval?}. These are stochastically sampled with temperature $t>0$ \jb{temperature is a technical detail not for here. sampled means stochastically by definition so no need to say that}. Contrast to 
\jb{I am unaware that `contrast to' is English} past approaches \cite{wang2023selfconsistency, Li2022OnTA} we use a separate \jb{dedicate} \entailment{} model to answer $q$. 
The \entailment{} receives as input $q$ and uniquely, a context which consists of the $k$ sampled chain \jb{chains?}, in \jb{the} order of their generation \jb{isn't the order completely random? there is no ordering except for time right? maybe we can just imagine it's a fixed random order?} \jb{it does seem pretty ridiculous that the input to entailment is a question and context and not premise and hypothesis...}. Each chain is expressed as a list of statements comprised solely of the intermediate QA pairs \jb{unclear how statements are qa pairs - maybe say it's just the qa pair?}. Fig.~\ref{fig:architecture} presents an example context \bb{the word context for entailment is perhaps a bit confusing and overloaded} (in pink \bb{background}) where each statement corresponds to a pair $(q_i, a_i)$ from chain $d^{(j)}$. Given the context, the \entailment{} model is prompted to generate the final answer to $q$ in chain-of-thought style \jb{what is chain-of-thought style? unclear what you mean by style and what it entails. Again, one wonders what are the prompts}. Namely, it first generates an explanation summarizing the key facts from the context which is followed by the final answer to $q$ (both in bold at the bottom of Fig.~\ref{fig:architecture}). This essentially equates to performing chain-of-thought reasoning in a reading comprehension setting, where the context itself is comprised of multiple chains of thought sampled from the \decomposition{} model. \jb{need to stress advantages again since your core point} 

\begin{figure}[t]\setlength{\belowcaptionskip}{-8pt}
  \centering
  \includegraphics[trim={0cm 1cm 0cm 0cm}, clip, width=0.92\textwidth]{figures/fig_decomp_retrieve.pdf}
  \vspace*{-0.7cm}
  \caption{Interleaving decomposition and retrieval steps. \oy{Do we want to add retrieval to the original question?} \jb{why no box saying `retrieval step \#2'?}}
  \label{fig:decompose_retrieve}
\end{figure}

